ADCB: An Alzheimer's disease benchmark for evaluating observational estimators of causal effects

Simulators make unique benchmarks for causal effect estimation since they do not rely on unverifiable assumptions or the ability to intervene on real-world systems, but are often too simple to capture important aspects of real applications. We propose a simulator of Alzheimer's disease aimed at modeling intricacies of healthcare data while enabling benchmarking of causal effect and policy estimators. We fit the system to the Alzheimer's Disease Neuroimaging Initiative (ADNI) dataset and ground hand-crafted components in results from comparative treatment trials and observational treatment patterns. The simulator includes parameters which alter the nature and difficulty of the causal inference tasks, such as latent variables, effect heterogeneity, length of observed history, behavior policy and sample size. We use the simulator to compare estimators of average and conditional treatment effects.

==> backup.tex <==
\section{Benchmarking causal effect estimators} \hltodo{FJ: Merge into 2 paragraphs of the introduction. Keep definitions of ATE and CATE and mention assumptions. }
Estimating causal effects from data is a central problem in machine learning and statistics\hltodo{cite}. The problem is well described using the language of potential outcomes~\citep{...}. Consider selecting an action $a$ from the (discrete) set $\mathcal{A} = \{0, 1, ..., k-1\}$. The \emph{potential outcome} that \emph{would be observed} under $a$ is denoted $Y(a)$. If we were to perform another action $b \in \mathcal{A}$, we would see potential outcome $Y(b)$. In this work, we let $A=0$ represent the special action of doing nothing. The difference between performing $a$ and doing nothing is often called the causal effect of $a$, defined as follows, 
$$
\Delta(a) = Y(a) - Y(0)~.
$$
Knowing the causal effect lets us assess the value of performing action $a$ and compare it to other actions. Now, consider estimating $\Delta$ using $m$ i.i.d. observations of actions and outcomes $(a_1, y_1), ..., (a_m, y_m) \sim p^m(A, Y)$. Only the outcome $Y=Y(A)$ of the performed action $A$ is observed for any one sample---not the causal effect. We must reason about what would happen if another action was chosen. 
%
In practice, potential outcomes $Y(a)$ are often stochastic and depend on more variables than the chosen action. Consequently, the effect $\Delta$ is identifiable from data only under very strict assumptions\hltodo{cite}. Instead, it is common to estimate aggregates over a distribution such as the average treatment effect (ATE)
$$
\tau(a) = \mathbb{E}[\Delta(a)]
$$
or conditional average treatment effects (CATE) with respect to a context $x$, 
$$
\tau(a \mid x) = \mathbb{E}[\Delta(a) \mid X=x]~.
$$
The quantities $\tau(a)$ and $\tau(a \mid x)$ represent the expected effects of performing action $a$ overall and conditioned on a context $x$, respectively. We refer to e.g.,\hltodo{...} for an in-depth discussion on estimation of these. The following assumptions are sufficient for consistent and unbiased estimation of ATE and CATE from observational data~\citep{...}.
\begin{thmasmp}[Identifying assumptions.]\label{asmp:identifiability}
Actions $A \in \mathcal{A}$, outcomes $Y \in \mathbb{R}$, a set of context variables $X$, and an adjustment set of variables $C \subseteq X$ are observed from a distribution $p(X,A,Y)$ such that the following conditions hold. 
\begin{align*}
\begin{array}{lll}
\mbox{{\bf Consistency}} &  Y = Y(A) & \\[1ex]
\mbox{{\bf Exchangeability}} & Y(a) \indep A \mid C, & \forall a\in \mathcal{A} \\[1ex]
\mbox{{\bf Overlap}} & p(A=a \mid C=c) > 0, & \forall a\in \mathcal{A}, c\in \mathcal{C}
\end{array}
\end{align*}
\end{thmasmp}%
Assumption~\ref{asmp:identifiability} is often made in theoretical analysis of causal effect estimation, but its validity is rarely known in practice. What is worse, consistency and exchangeability cannot be verified from data~\citep{...}. Moreover, the assumptions do not guarantee good estimates when sample sizes are small. For these reason, central questions when comparing effect estimators are: How well do they perform when the identifying assumptions are violated? How much do they rely on large sample sizes? A good benchmark should help to answer these questions. \hltodo{Comment on realistic violations/sample sizes}

\hltodo{Talk about sequential data here?}










Alzheimer's disease (AD) is the most common form of dementia, affecting tens of millions of people worldwide~\citep{AlzAsso}. Despite its toll on public health and vast research investments over several decades, there is currently no drug available that cures AD. Nevertheless, drugs that have disease-modifying effects, alleviating symptoms such as loss of cognitive function, have shown promise in trials and in practice~\citep{grossberg2019present}. For these reasons and more, AD makes a good setting for benchmarking causal effect estimators:

\begin{itemize}
    \item AD is a progressive disorder, deteriorating the health of subjects over time. As a result, data is often collected for the same subjects at several time points, allowing for comparing the performance of longitudinal models of causal effects.
    \item There is evidence that AD is not a single disease but a group of multiple disease subtypes. While the precise nature of this is still unknown, disease subtypes provide a potentially challenging source of heterogeneity in patient outcomes.
    \item Most current treatments are believed to be symptomatic---they affect only symptoms and not the underlying disease cause; their effects disappear once discontinued. This allows for easier attribution of effect to treatment.
\end{itemize}








%
% Evaluation for data fidelity
%
\section{Evaluation of the benchmark}
\label{sec:evaluation}
Although our emphasis is on building a simulator that has utility in evaluating causal effects, we also verify that the data generated from the simulator is realistic with respect to the original ADNI dataset. We do this both qualitatively and quantitatively; by visual inspection of the statistics of the data generated compared to the original data \hltodo{NM Histograms+ Visual--Gaussian Kernel density? as well as quantitatively with two-sample tests}. The following outline sample statistics from both sets of data for selected covariates; 
\\
%
\hltodo{Sample Histograms}
\hltodo{Table 1}
\hltodo{How well do we fit the data?}







%
% Related work
%
\section{Related work}
\label{sec:related}
\hltodo{FJ: Cut or move to the appendix}
Benchmarking effect estimators is a central problem in causal inference~\citep{wendling2018comparing,shimoni2018benchmarking,gentzel2019case,dorie2019automated,gentzel2021and}. The possibility of producing confounded evaluation metrics prevents using only observational data for this task, without relying on strong assumptions. There are two main approaches which do not rely on such assumptions: a) making use of data from randomized experiments, and b) simulating all or part the system under investigation. See~\citet{gentzel2019case} for an excellent discussion of the pros and cons of each approach. Making use of as much real data for simulation as possible is also called the Empirical Monte Carlo Study (EMCS) approach~\citep{huber2013performance,lechner2013sensitivity}.

Data from randomized experiments are free from confounding bias, which allows for unbiased estimation of causal effects under the (often plausible) assumption of consistency~\citep{gentzel2021and}. To construct a non-trivial benchmark from such data, confounding bias is typically introduced by adding or subsampling data in ways which depend on the contexts of interventions~\citep{hill2011bayesian,kallus2018removing,zhang2021bounding}. The IHDP~\citep{hill2011bayesian} dataset introduces confounding by removing a biased subset of subjects. The famous LaLonde randomized experiment~\citep{lalonde1986evaluating} has been used as a benchmark after mixing in observational (potentially selection-biased) samples~\citep{smith2005does,shalit2017estimating} in the data accessed by estimators. Only the experimental portion is then used for evaluation. Yet another approach is to sample new treatment assignments for study subjects, keeping only the subset of them which agree with the observations from the experiment~\citep{louizos2017causal}. 

A great benefit of using experimental data for evaluation is that it only requires simulating a new treatment assignment policy if the goal is to estimate average treatment effects or the average value of treatment policies~\citep{gentzel2021and}. This is often preferred over simulating the outcome, since treatment policies are within human control, but outcome mechanisms typically are not. Standard or weighted Monte-Carlo estimates are sufficient for evaluation in this case. Drawbacks of this approach include that individual-level counterfactuals and effects remain unknown, and that the sample size is limited to the number of experiment subjects.

If the goal of a benchmark is to evaluate individual-level or fine conditional treatment effects, access to counterfactual outcomes is required. The only way to reliably achieve this is to simulate the mechanism determining the outcome of interventions, which can be done in isolation or in addition to simulating the treatment assignment, as in the Causal Inference Benchmarking Framework by \citet{shimoni2018benchmarking}, the Medkit-Learning environment (focused on reinforcement learning)~\citep{chan2021medkit}, and in IHDP~\citep{hill2011bayesian}. Since the outcome mechanisms are often the main target of estimation, these simulations should be as realistic as possible for the domain they aim to represent. To this end, researchers have considered building their simulators on models fit to observational data~\citep{neal2020realcause,chan2021medkit}.

A drawback of simulated data is that, in many cases, simulators ``tend to match the assumptions of the researcher''~\citep{gentzel2019case}. This is especially problematic in cases where they are introduced to evaluate one particular estimator which may also match those assumptions. As a result, it is important that simulator-based benchmarks contain settings that break or tweak assumptions to appropriately test the robustness of estimators to these. % still have the researcher degrees-of-freedom problem
\hltodo{we're leaning a bit too heavily on Gentzel 2019, 2020 at the moment.}
